Analysis of the spatially-resolved $V$-3.6$\mu$m colors and dust extinction in 257 nearby NGC and IC galaxies

We present and analyze spatially-resolved maps for the observed $V$- and $g$-band to 3.6$\mu$m flux ratios and the inferred dust extinction values, $A_V$, for a sample of 257 nearby NGC and IC galaxies. Flux ratio maps are constructed using PSF-matched mosaics of SDSS $g$- and $r$-band images and Spitzer/IRAC 3.6$\mu$m mosaics, with all pixels contaminated by foreground stars or background objects masked out. By applying the $\beta_V$ method (Tamura et al. 2009, 2010), which was recently calibrated as a function of redshift and morphological type by Kim, Jansen, & Windhorst (2017), dust extinction maps were created for each galaxy. The typical 1-$\sigma$ scatter in $\beta_V$ around the average, both within a galaxy and in each morphological type bin, is $\sim$20%. Combined, these result in a $\sim$0.4 mag scatter in $A_V$. $\beta_V$ becomes insensitive to small-scale variations in stellar populations once resolution elements subtend an angle larger than that of a typical giant molecular cloud ($\sim$200pc). We find noticeably redder $V$$-$3.6$\mu$m colors in the center of star-forming galaxies and galaxies with a weak AGN. The derived intrinsic $V$$-$3.6$\mu$m colors for each Hubble type are generally consistent with the model predictions of Kim et al. (2017). Finally, we discuss the applicability of the $\beta_V$ dust-correction method to more distant galaxies, for which well-matched HST rest-frame visible and JWST rest-frame $\sim$3.5$\mu$m images will become available in the near-future.

==> table1.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%  TABLE 1: The list of 257 NGC/IC galaxies sample
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\clearpage
\setlength{\tabcolsep}{2pt}
\startlongtable
\begin{deluxetable*}{lccccccccrccccccccccl}
\tabletypesize{\scriptsize}
\tablecolumns{21}
%\tablewidth{7in}
%\tablenum{1}
\tablecaption{The list of NGC/IC galaxy sample} 
%\tablecaption{Nearby galaxies imaged with WFPC2 in the mid-UV in
%              Cycle~9\,$\string^a$\label{Table-1}} 
\tablehead{
% --- first line of table header:
\colhead{ID}    & \colhead{R.A.(J2000)}		& \colhead{Decl.(J2000)}		&
\colhead{$z$}		& \colhead{$B$}		& \colhead{$V$}			&
\colhead{3.6\micron} & \colhead{3.6\micron}	& \colhead{$a$}		& \colhead{$b/a$} 	& \colhead{r$_{\mathrm{eff}}$}	& \colhead{$R_{50,V}^{P}$}		& \colhead{PA}		& \colhead{Gal. Ext.}	& \colhead{B/T}		& 
\colhead{T} 		& \colhead{eT}		& \colhead{Type}			& 
\colhead{SF \&}	& \colhead{Classification}	& \colhead{Figure}\\ 
% --- second line of table header:
\colhead{}         	& \colhead{(deg)}    & \colhead{(deg)}		&
\colhead{}          & \colhead{(mag)}  	& \colhead{(mag)} 			&
\colhead{(mag)}		& \colhead{(Mag)}	& \colhead{(\arcmin)} 		& \colhead{}			& \colhead{(\arcsec)} & \colhead{(\arcsec)}		& \colhead{(deg)}		& \colhead{(mag)}	& \colhead{}				& 
\colhead{}        	& \colhead{}		& \colhead{}			&	 
\colhead{AGN}        	& \colhead{}			& \colhead{Set 2 \#}\\ 
% --- third line of table header
\colhead{(1)}          & \colhead{(2)}        & \colhead{(3)}       &
\colhead{(4)}          & \colhead{(5)}        & \colhead{(6)}       &
\colhead{(7)}          & \colhead{(8)}        & \colhead{(9)} 		&
\colhead{(10)}          & \colhead{(11)}        & \colhead{(12)} 	&
\colhead{(13)}          & \colhead{(14)}        & \colhead{(15)} 	&
\colhead{(16)}		& \colhead{(17)}	& \colhead{(18)}			&
\colhead{(19)}		& \colhead{(20)}	& \colhead{(21)}
}
\startdata
%----
NGC 0014 &   2.193333 &  15.815556 & 0.002885 & 12.7 & 12.1 & 12.7 & --17.8 & 2.8 & 0.75 &  44.4 & 24.0 & 25.0 & 0.117 & 0.19 & 10.0 & 0.3 & IBm & 0 & (R)IB(s)m pec & 1 \\ 
NGC 0023 &   2.472542 &  25.923778 & 0.015231 & 12.9 & 12.0 & 11.5 & --22.7 & 2.1 & 0.62 &  14.4 &  4.2 & 8.0 & 0.145 & 0.49 & 1.0 & 0.4 & SBa & 2 & SB(s)a;HII;LIRGSbrst & 2 \\ 
NGC 0193 &   9.827458 &   3.331111 & 0.014723 & 13.3 & 12.3 & 11.7 & --22.4 & 1.4 & 0.86 &  19.5 & 13.8 & 55.0 & 0.061 & 0.78 & --2.5 & 0.6 & E/SB0 & 0 & SAB(s)0-: & 3 \\ 
NGC 0266 &  12.449167 &  32.277722 & 0.015547 & 12.5 & 11.6 & 10.3 & --23.9 & 3.0 & 0.97 &  42.3 & 31.2 & 99.0 & 0.217 & 0.28 & 2.0 & 0.7 & SBab & 3 & SB(rs)ab       LINER & 4 \\ 
NGC 0274 &  12.757750 & --7.056944 & 0.005837 & 12.8 & 11.8 & 11.7 & --20.3 & 1.5 & 1.00 & * &  7.8 & 25.0 & 0.211 & 0.45 & --3.0 & 0.4 & E/SB0 & 0 & SAB(r)0- pec & 5 \\ 
NGC 0275 &  12.767500 & --7.066667 & 0.005817 & 13.2 & 12.5 & 12.3 & --19.8 & 1.5 & 0.73 & * & 18.0 & 126.0 & 0.211 & 0.00 & 6.0 & 0.4 & SBcd/P & 0 & SB(rs)cd pec & 6 \\ 
NGC 0309 &  14.177750 & --9.913861 & 0.018886 & 12.5 & 11.9 & 11.8 & --22.9 & 1.94 & 0.69 &  44.4 & 31.2 & 175.0 & 0.156 & 0.06 & 5.0 & 0.3 & SBc & 0 & SAB(r)c        HII & 7 \\ 
NGC 0315 &  14.453667 &  30.352444 & 0.016485 & 12.2 & 11.2 & 10.3 & --24.0 & 2.08 & 0.74 &  36.9 & 23.4 & 43.0 & 0.261 & 0.78 & --4.0 & 0.5 & E2 & 5 & E+:;LINER;Sy3b Sy1 & 8 \\ 
NGC 0337 &  14.958708 & --7.577972 & 0.00549 & 12.1 & 11.6 & 11.0 & --21.0 & 2.9 & 0.62 &  31.5 & 25.8 & 141.0 & 0.316 & 0.31 & 7.0 & 0.3 & SBcd & 0 & SB(s)d         HII & 9 \\ 
NGC 0382 &  16.849458 &  32.403861 & 0.017442 & 14.2 & 13.2 & 12.3 & --22.2 & 0.7 & 1.00 & * &  5.4 & * & 0.173 & 0.61 & --5.0 & 0.5 & E0 & 0 & E:             HII & 10 \\ 
NGC 0383 &  16.854000 &  32.412556 & 0.017005 & 13.2 & 12.2 & 10.8 & --23.6 & 1.6 & 0.87 & * & 15.0 & 30.0 & 0.173 & 0.75 & --3.0 & 0.3 & E-S0 & 5 & SA0-:;BrClG;Sy LERG & 11 \\ 
NGC 0410 &  17.745417 &  33.151889 & 0.017659 & 12.5 & 11.5 & 11.0 & --23.5 & 2.4 & 0.54 &  34.5 & 16.2 & 30.0 & 0.189 & 0.55 & --4.0 & 0.6 & cD & 3 & E+:;LINER      HII & 12 \\ 
NGC 0428 &  18.232125 &   0.981556 & 0.003843 & 11.9 & 11.5 & 12.2 & --19.0 & 4.1 & 0.76 &  49.8 & 34.2 & 120.0 & 0.025 & 0.00 & 9.0 & 0.3 & SBm & 0 & SAB(s)m        HII & 13 \\ 
NGC 0507 &  20.916292 &  33.256056 & 0.016458 & 12.2 & 11.2 & 10.5 & --23.9 & 3.1 & 1.00 &  53.4 & 37.8 & * & 0.165 & 0.39 & --2.0 & 0.3 & E-S0 & 0 & SA(r)0\string^0\string^;BrClG & 14 \\ 
NGC 0514 &  21.016250 &  12.917389 & 0.008246 & 12.2 & 11.7 & 11.7 & --21.1 & 3.5 & 0.80 &  65.7 & 36.0 & 110.0 & 0.073 & 0.03 & 5.0 & 0.3 & SBc & 0 & SAB(rs)c & 15 \\ 
NGC 0596 &  23.217000 & --7.031833 & 0.006258 & 11.8 & 10.9 & 10.6 & --21.7 & 3.2 & 0.66 &  27.3 & 16.8 & 40.0 & 0.107 & 0.62 & --4.0 & 0.5 & E4 & 0 & E+ pec: & 16 \\ 
NGC 0636 &  24.777208 & --7.512611 & 0.006204 & 12.4 & 11.5 & 11.0 & --21.2 & 2.8 & 0.75 &  19.5 & 10.8 & 40.0 & 0.119 & 0.61 & --5.0 & 0.3 & E3 & 0 & E3 & 17 \\ 
NGC 0695 &  27.809333 &  22.582361 & 0.032472 & 13.8 & 12.8 & 11.6 & --24.2 & 0.8 & 0.87 & * &  6.0 & 40.0 & 0.297 & 0.68 & --2.0 & 1.9 & S0/P & 2 & S0? pec;LIRG   HII & 18 \\ 
NGC 0741 &  29.087625 &   5.628944 & 0.018549 & 12.2 & 11.1 & 10.8 & --23.8 & 3.0 & 0.97 &  52.2 & 25.2 & 90.0 & 0.133 & 0.81 & --5.0 & 0.4 & E0 & 0 & E0: & 19 \\ 
NGC 0772 &  29.831583 &  19.007528 & 0.008246 & 11.1 & 10.3 &  9.5 & --23.4 & 7.2 & 0.60 &  77.1 & 43.2 & 130.0 & 0.157 & 0.24 & 3.0 & 0.3 & Sb & 0 & SA(s)b         HII & 20 \\ 
NGC 0777 &  30.062083 &  31.429583 & 0.016728 & 12.5 & 11.5 & 11.0 & --23.4 & 2.5 & 0.80 &  34.5 & 11.4 & 155.0 & 0.145 & 0.66 & --5.0 & 0.3 & E1 & 3 & E1          Sy;LINER & 21 \\ 
NGC 0788 &  30.276875 & --6.815528 & 0.013603 & 13.0 & 12.1 & 11.6 & --22.3 & 1.9 & 0.74 &  17.7 & 12.0 & 111.0 & 0.067 & 0.21 & -.0 & 0.6 & S0-a & 5 & SA(s)0/a:;Sy1  Sy2 & 22 \\ 
IC 0195 &  30.935875 &  14.709278 & 0.012168 & 14.0 & 13.0 & 12.7 & --21.0 & 1.17 & 0.51 & * &  3.6 & 126.0 & 0.137 & 0.72 & --2.0 & 0.8 & S0 & 0 & SAB0\string^0\string^ & 23 \\ 
IC 0208 &  32.115583 &   6.394917 & 0.011755 & 14.2 & 13.4 & 12.9 & --20.7 & 1.8 & 1.00 & * & 19.8 & * & 0.133 & 0.03 & 4.0 & 0.8 & Sbc & 0 & SAbc & 24 \\ 
IC 0214 &  33.523292 &   5.173250 & 0.030224 & 14.7 & 14.2 & 11.3 & --24.4 & 0.8 & 0.75 & * &  3.0 & 162.0 & 0.109 & 0.18 & 7.0* & * & Sd & 2 & I?             LIRG & 25 \\ 
NGC 0985 &  38.657375 & --8.787611 & 0.043143 & 14.0 & 13.4 & 12.8 & --23.6 & 1.0 & 0.90 &  13.2 &  8.4 & 69.0 & 0.093 & 0.73 & 10.0 & 0.8 & Ring/P & 5 & SBbc? p (Ring) Sy1 & 26 \\ 
NGC 0992 &  39.356208 &  21.100833 & 0.013813 & 13.7 & 12.8 & 11.6 & --22.3 & 0.9 & 0.78 & * &  5.4 & 7.0 & 0.409 & 0.45 & 5.0* & * & Sc & 2 & S?             LIRG & 27 \\ 
NGC 1016 &  39.581500 &   2.119250 & 0.022209 & 12.6 & 11.6 & 11.0 & --24.0 & 2.4 & 1.00 &  36.0 & 19.2 & * & 0.053 & 0.69 & --4.5 & 0.5 & E0 & 0 & E & 28 \\ 
NGC 1143 &  43.790458 & --0.177861 & 0.028216 & 14.1 & 13.1 & 12.5 & --23.0 & 0.9 & 0.89 & * &  8.4 & 110.0 & 0.177 & 0.29 & --4.3 & 0.6 & Ring A & 0 & S0 pec (Ring A) & 29 \\ 
NGC 1144 &  43.800833 & --0.183556 & 0.028847 & 13.8 & 13.0 & 12.0 & --23.6 & 1.1 & 0.64 &  16.8 &  9.0 & 130.0 & 0.177 & 0.40 & 3.0* & * & Ring B & 4 & S pec (Ring B) Sy2 & 30 \\ 
NGC 1265 &  49.565250 &  41.857750 & 0.025137 & 14.4 & 13.4 & 11.3 & --24.0 & 1.8 & 0.89 &  41.4 & 12.0 & 125.0 & 0.753 & 0.66 & --4.0 & 0.5 & E5 & 0 & E+             LERG & 31 \\ 
NGC 1275 &  49.950667 &  41.511694 & 0.017559 & 12.6 & 11.9 & 10.8 & --23.7 & 2.2 & 0.77 &  16.8 & 22.2 & 110.0 & 0.697 & 0.29 & 99.0 & * & S0/P & 4 & cD;pec;NLRG;Sy2;LEG & 32 \\ 
NGC 1667 &  72.154750 & --6.319972 & 0.015167 & 12.8 & 12.1 & 11.4 & --22.8 & 1.8 & 0.78 &  18.6 & 12.6 & 20.0 & 0.221 & 0.05 & 5.0 & 0.4 & SBc & 4 & SAB(r)c        Sy2 & 33 \\ 
NGC 1700 &  74.234625 & --4.865778 & 0.012972 & 12.2 & 11.2 & 10.5 & --23.3 & 3.3 & 0.64 &  18.6 &  9.0 & 120.0 & 0.113 & 0.82 & --5.0 & 0.3 & E4 & 0 & E4 & 34 \\ 
NGC 2403 & 114.214167 &  65.602556 & 0.000445 & 8.9 & 8.5 &  8.6 & --17.9 & 21.9 & 0.56 & 143.7 & 126.0 & 127.0 & 0.157 & 0.00 & 6.0 & 0.3 & SBc & 3 & SAB(s)cd;HII   LINER & 35 \\ 
NGC 2415 & 114.236208 &  35.241972 & 0.012622 & 12.8 & 12.4 & 11.6 & --22.2 & 0.9 & 1.00 & * &  7.2 & * & 0.161 & 0.37 & 10.0 & 1.7 & Im & 0 & Im? & 36 \\ 
IC 0486 & 120.087417 &  26.613528 & 0.026875 & 14.6 & 13.7 & 12.6 & --22.8 & 1.11 & 0.66 & * &  6.0 & 139.0 & 0.049 & 0.59 & 1.0 & 0.9 & SBa & 5 & Sy1 & 37 \\ 
NGC 2500 & 120.471708 &  50.737111 & 0.001681 & 12.2 & 11.6 & 11.1 & --18.2 & 2.9 & 0.90 & * & 40.8 & 48.0 & 0.129 & 0.21 & 7.0 & 0.3 & SBcd & 0 & SB(rs)d        HII & 38 \\ 
NGC 2512 & 120.782708 &  23.391833 & 0.015684 & 13.9 & 13.1 & 12.3 & --21.9 & 1.4 & 0.64 &  12.9 & 11.4 & 113.0 & 0.161 & 0.31 & 3.0 & 0.8 & SBb & 1 & SBb            Sbrst & 39 \\ 
IC 2239 & 123.528292 &  23.866361 & 0.020174 & 14.6 & 13.6 & 12.9 & --21.9 & 1.3 & 0.85 & * &  4.8 & 168.0 & 0.185 & 0.46 & 0.0* & * & S0 & 0 & S0? & 40 \\ 
NGC 2552 & 124.835542 &  50.009639 & 0.001748 & 12.6 & 12.1 & 13.1 & --16.4 & 3.5 & 0.66 &  68.7 & 43.2 & 57.0 & 0.165 & 0.00 & 9.0 & 0.3 & SBm & 0 & SA(s)m? & 41 \\ 
IC 0505 & 125.840292 &   4.372472 & 0.031232 & 14.9 & 14.0 & 12.9 & --22.9 & 1.24 & 0.69 & * &  9.6 & 143.0 & 0.033 & 0.23 & 3.0* & * & S & 5 & S;BrClG        AGN & 42 \\ 
NGC 2604 & 128.346417 &  29.538806 & 0.00693 & 13.3 & 12.6 & 13.0 & --19.5 & 2.1 & 1.00 & * & 25.2 & * & 0.105 & 0.14 & 6.0 & 0.8 & SBc & 1 & SB(rs)cd;WR;HIISbrst & 43 \\ 
NGC 2608 & 128.822208 &  28.473417 & 0.007122 & 13.0 & 12.3 & 11.5 & --21.0 & 2.3 & 0.61 &  25.5 & 18.6 & 60.0 & 0.109 & 0.09 & 3.0 & 0.5 & SBb & 0 & SB(s)b: & 44 \\ 
NGC 2685 & 133.894625 &  58.734389 & 0.002945 & 12.1 & 11.3 & 10.9 & --19.6 & 4.5 & 0.51 &  32.1 & 10.2 & 38.0 & 0.149 & 0.76 & --1.0 & 0.3 & SB0-a & 4 & (R)SB0+ pec;RETSy2 & 45 \\ 
NGC 2712 & 134.876958 &  44.913889 & 0.006054 & 12.8 & 12.1 & 11.3 & --20.9 & 2.9 & 0.55 &  27.9 & 18.6 & 178.0 & 0.037 & 0.15 & 3.0 & 0.5 & SBb & 0 & SB(r)b: & 46 \\ 
NGC 2731 & 135.535042 &   8.301667 & 0.008616 & 14.4 & 13.7 & 12.9 & --20.0 & 0.8 & 0.62 & * &  7.2 & 70.0 & 0.177 & 0.11 & 5.0* & * & Sc & 0 & S? & 47 \\ 
NGC 2730 & 135.565958 &  16.838306 & 0.012782 & 13.6 & 13.0 & 12.5 & --21.3 & 1.7 & 0.76 & * & 19.8 & 80.0 & 0.077 & 0.09 & 8.0 & 1.1 & SBdm & 0 & SBdm: & 48 \\ 
NGC 2750 & 136.449625 &  25.437417 & 0.00892 & 12.6 & 11.9 & 11.7 & --21.3 & 1.9 & 0.79 & * & 30.6 & 81.0 & 0.133 & 0.22 & 5.0 & 0.7 & Sc & 0 & Sc & 49 \\ 
NGC 2740 & 136.520792 &  51.735306 & 0.029516 & 14.8 & 14.0 & 14.2 & --21.4 & 0.76 & 0.83 & * &  8.4 & 45.0 & 0.017 & 0.21 & 2.0* & * & Sab & 4 & S?             NLAGN & 50 \\ 
NGC 2742 & 136.889708 &  60.479333 & 0.0043 & 12.0 & 11.4 & 10.8 & --20.6 & 3.0 & 0.50 &  45.3 & 28.2 & 87.0 & 0.185 & 0.00 & 5.0 & 0.5 & Sc & 0 & SA(s)c: & 51 \\ 
NGC 2768 & 137.906250 &  60.037222 & 0.004513 & 10.8 & 9.9 &  9.6 & --21.9 & 8.1 & 0.53 &  64.2 & 24.0 & 95.0 & 0.161 & 0.61 & --5.0 & 0.3 & E6 & 3 & S0\_1/2\_        LINER & 52 \\ 
NGC 2776 & 138.060458 &  44.954833 & 0.008759 & 12.1 & 11.6 & 11.6 & --21.3 & 2.32 & 0.62 &  33.6 & 24.0 & 0.0 & 0.037 & 0.09 & 5.0 & 0.3 & SBc & 0 & SAB(rs)c & 53 \\ 
NGC 2778 & 138.101542 &  35.027528 & 0.006835 & 13.4 & 12.4 & 12.1 & --20.3 & 1.4 & 0.71 &  15.6 &  7.8 & 40.0 & 0.021 & 0.39 & --5.0 & 0.8 & E3 & 0 & E & 54 \\ 
NGC 2782 & 138.521292 &  40.113694 & 0.008483 & 12.3 & 11.6 & 11.3 & --21.6 & 3.5 & 0.74 &  23.4 & 19.8 & 74.0 & 0.0 & 0.55 & 1.0 & 0.3 & SBa & 5 & SAB(rs)a;Sy1   Sbrst & 55 \\ 
NGC 2824 & 139.759292 &  26.269972 & 0.0092 & 14.2 & 13.3 & 12.6 & --20.5 & 0.9 & 0.67 &   6.6 &  3.6 & 160.0 & 0.061 & 0.51 & --2.0 & 0.9 & S0 & 4 & S0             Sy? & 56 \\ 
NGC 2831 & 139.939542 &  33.745000 & 0.017279 & 14.3 & 13.3 & 12.3 & --22.2 & 0.71 & 0.73 & * &  5.4 & * & 0.0 & 0.27 & --5.0 & 0.5 & E0 & 0 & E0 & 57 \\ 
NGC 2832 & 139.945250 &  33.749750 & 0.023176 & 12.9 & 11.9 & 11.4 & --23.7 & 1.71 & 0.69 &  25.5 & 12.0 & 160.0 & 0.0 & 0.73 & --4.0 & 0.3 & E2 & 3 & E+2:;cD        LINER & 58 \\ 
NGC 2844 & 140.450042 &  40.151250 & 0.004957 & 13.8 & 13.0 & 12.5 & --19.3 & 1.5 & 0.53 & * &  8.4 & 13.0 & 0.0 & 0.46 & 1.0 & 0.6 & Sa & 0 & SA(r)a:        HII & 59 \\ 
NGC 2893 & 142.570667 &  29.539972 & 0.005667 & 13.9 & 13.2 & 12.8 & --19.2 & 1.1 & 0.91 & * &  3.6 & 79.0 & 0.021 & 0.41 & -.0 & 0.8 & SB0-a & 1 & (R)SB0/a       Sbrst & 60 \\ 
NGC 2906 & 143.025917 &   8.441778 & 0.007138 & 13.4 & 12.7 & 11.5 & --21.0 & 1.4 & 0.64 & * & 12.0 & 75.0 & 0.073 & 0.09 & 6.0 & 1.2 & Sc & 0 & Scd: & 61 \\ 
NGC 2892 & 143.220542 &  67.617389 & 0.022822 & 14.1 & 13.1 & 11.9 & --23.1 & 1.4 & 1.00 & * & 13.2 & * & 0.157 & 0.58 & --3.5 & 0.6 & E0 & 0 & E+ pec: & 62 \\ 
NGC 2937 & 144.437625 &   2.747361 & 0.022702 & 14.6 & 13.7 & 12.7 & --22.3 & 0.7 & 0.76 &   9.9 &  3.0 & 0.0 & 0.085 & 0.59 & --5.0 & 0.9 & E3 & 0 & E & 63 \\ 
IC 0559 & 146.182875 &   9.615000 & 0.001806 & 15.1 & 14.2 & 14.7 & --14.8 & 0.8 & 0.75 & * & 10.2 & 90.0 & 0.033 & 0.00 & 5.0* & * & S? & 0 & Sc & 64 \\ 
NGC 3015 & 147.345500 &   1.145417 & 0.025017 & 14.5 & 13.5 & 12.9 & --22.3 & 0.71 & 0.77 & * &  4.2 & 95.0 & 0.117 & 0.13 & --2.0 & 1.9 & S0 & 4 & SAB0\string^0\string^ pec?   NLAGN & 65 \\ 
NGC 3011 & 147.421667 &  32.221111 & 0.005147 & 14.3 & 13.3 & 13.6 & --18.2 & 0.96 & 0.76 & * &  4.2 & 69.0 & 0.013 & 0.39 & --2.0 & 0.9 & S0 & 0 & S0/a & 66 \\ 
NGC 3020 & 147.527500 &  12.813639 & 0.004803 & 12.6 & 11.9 & 13.5 & --18.2 & 3.2 & 0.50 & * & 21.6 & 105.0 & 0.017 & 0.06 & 6.0 & 0.5 & SBc & 0 & SB(r)cd: & 67 \\ 
NGC 3032 & 148.033958 &  29.236222 & 0.00521 & 13.2 & 12.5 & 12.2 & --19.7 & 2.0 & 0.90 &   9.3 &  2.4 & 95.0 & 0.021 & 0.39 & --2.0 & 0.3 & SB0 & 0 & SAB(r)0\string^0\string^     HII & 68 \\ 
NGC 3049 & 148.706500 &   9.271083 & 0.004854 & 12.9 & 12.1 & 11.8 & --19.9 & 2.13 & 0.50 & * & 24.6 & 25.0 & 0.037 & 0.24 & 2.0 & 0.8 & SBab & 1 & SB(rs)ab;HII   Sbrst & 69 \\ 
NGC 3055 & 148.825250 &   4.270028 & 0.006021 & 12.7 & 12.1 & 11.9 & --20.2 & 2.12 & 0.57 & * & 16.8 & 63.0 & 0.093 & 0.12 & 5.0 & 0.4 & SBc & 0 & SAB(s)c        WR & 70 \\ 
IC 2520 & 149.083833 &  27.227583 & 0.00413 & 14.4 & 13.4 & 12.4 & --18.9 & 0.83 & 0.89 & * &  7.2 & 90.0 & 0.033 & 0.27 & 99.0 & * & P & 0 & Pec            HII & 71 \\ 
IC 2551 & 152.668000 &  24.414139 & 0.021185 & 14.4 & 13.6 & 12.9 & --22.0 & 0.87 & 0.78 & * &  1.8 & 33.0 & 0.105 & 0.55 & 3.0* & * & S & 0 & S?             WR? & 72 \\ 
NGC 3162 & 153.381625 &  22.737556 & 0.00433 & 12.2 & 11.6 & 11.9 & --19.5 & 3.0 & 0.83 &  34.5 & 25.2 & 33.0 & 0.065 & 0.10 & 4.0 & 0.3 & SBbc & 0 & SAB(rs)bc & 73 \\ 
NGC 3184 & 154.570250 &  41.424056 & 0.001975 & 10.4 & 9.8 &  8.9 & --20.8 & 7.4 & 0.93 & 116.7 & 91.2 & 135.0 & 0.0 & 0.04 & 6.0 & 0.3 & SBc & 0 & SAB(rs)cd      HII & 74 \\ 
NGC 3192 & 154.771375 &  46.454111 & 0.030721 & 14.1 & 13.3 & 13.3 & --22.4 & 0.8 & 0.75 & * &  7.8 & 5.0 & 0.0 & 0.08 & 4.0* & * & SBbc/P & 0 & SB(s)bc pec & 75 \\ 
NGC 3239 & 156.270375 &  17.163583 & 0.002512 & 11.7 & 11.3 &  8.5 & --21.7 & 5.0 & 0.66 &  36.9 & 52.2 & 81.0 & 0.105 & 0.07 & 10.0 & 0.3 & IBm/P & 0 & IB(s)m pec & 76 \\ 
NGC 3212 & 157.068583 &  79.823389 & 0.032402 & 14.0 & 13.2 & 13.6 & --22.2 & 1.1 & 0.91 & * &  6.6 & 92.0 & 0.013 & 0.48 & 3.0* & * & SBb & 0 & S? & 77 \\ 
NGC 3215 & 157.169083 &  79.813083 & 0.031582 & 13.9 & 13.1 & 12.5 & --23.3 & 1.5 & 0.73 & * & 12.0 & 52.0 & 0.013 & 0.14 & 4.0* & * & Sbc & 0 & SB? & 78 \\ 
NGC 3265 & 157.778208 &  28.796667 & 0.0044 & 13.9 & 12.9 & 12.8 & --18.6 & 0.96 & 0.70 & * &  4.8 & 73.0 & 0.053 & 0.66 & --5.0 & 0.7 & E2 & 0 & E:;WR?         HII & 79 \\ 
NGC 3310 & 159.691083 &  53.503389 & 0.003312 & 11.2 & 10.8 & 11.0 & --19.9 & 3.1 & 0.77 &  12.3 &  9.6 & 156.0 & 0.0 & 0.46 & 4.0 & 0.3 & SBbc/P & 0 & SAB(r)bc pec   HII & 80 \\ 
NGC 3319 & 159.789417 &  41.686667 & 0.002465 & 11.5 & 11.1 &  9.3 & --20.9 & 6.2 & 0.55 & 128.1 & 60.0 & 37.0 & 0.0 & 0.11 & 6.0 & 0.3 & SBc & 0 & SB(rs)cd       HII: & 81 \\ 
NGC 3344 & 160.879792 &  24.922222 & 0.001935 & 10.5 & 9.9 &  9.7 & --20.0 & 7.1 & 0.92 &  88.5 & 61.2 & 18.0 & 0.025 & 0.09 & 4.0 & 0.3 & SBbc & 0 & (R)SAB(r)bc    HII & 82 \\ 
NGC 3349 & 160.960667 &   6.762972 & 0.027536 & 15.2 & 14.5 & 14.1 & --21.4 & 0.65 & 0.97 & * &  5.4 & * & 0.053 & 0.19 & 5.0* & * & Sc & 0 & WR?            HII & 83 \\ 
NGC 3351 & 160.990417 &  11.703806 & 0.002595 & 10.5 & 9.7 &  7.3 & --23.0 & 3.07 & 0.93 &  64.2 & 60.0 & 13.0 & 0.045 & 0.13 & 3.0 & 0.3 & SBb & 1 & SB(r)b;HII     Sbrst & 84 \\ 
NGC 3370 & 161.766875 &  17.273611 & 0.004266 & 12.3 & 11.6 & 11.7 & --19.7 & 3.2 & 0.56 & * & 18.6 & 148.0 & 0.037 & 0.45 & 5.0 & 0.3 & Sc & 0 & SA(s)c & 85 \\ 
NGC 3381 & 162.103417 &  34.711417 & 0.005434 & 12.7 & 11.8 & 12.5 & --19.4 & 1.46 & 0.96 & * & 19.8 & 60.0 & 0.0 & 0.29 & 5.0* & * & SB/P & 0 & SB pec;WR      HII & 86 \\ 
NGC 3395 & 162.458792 &  32.982861 & 0.00542 & 12.4 & 12.1 & 12.2 & --19.7 & 2.1 & 0.57 & * & 12.6 & 50.0 & 0.0 & 0.15 & 6.0 & 0.6 & SBc & 0 & SAB(rs)cd pec: HII & 87 \\ 
NGC 3414 & 162.817542 &  27.975111 & 0.004903 & 12.0 & 11.0 & 10.6 & --21.1 & 3.5 & 0.74 &  20.7 & 13.8 & 25.0 & 0.0 & 0.56 & --2.0 & 0.3 & SB0 & 3 & S0 pec         LINER & 88 \\ 
NGC 3419 & 162.823917 &  13.946000 & 0.010124 & 13.4 & 12.5 & 12.6 & --20.6 & 1.2 & 0.83 & * &  4.2 & 115.0 & 0.045 & 0.47 & --1.0 & 0.5 & SB0-a & 0 & (R)SAB(r)0+ & 89 \\ 
NGC 3489 & 165.077375 &  13.901222 & 0.002258 & 11.1 & 10.3 & 10.0 & --20.0 & 3.5 & 0.57 &  20.4 &  9.0 & 70.0 & 0.021 & 0.57 & --1.0 & 0.3 & SB0-a & 3 & SAB(rs)0+   Sy;LINER & 90 \\ 
NGC 3486 & 165.099458 &  28.975139 & 0.002272 & 11.1 & 10.5 & 10.6 & --19.4 & 7.1 & 0.73 &  62.7 & 39.0 & 80.0 & 0.015 & 0.41 & 5.0 & 0.3 & SBc & 4 & SAB(r)c;HII    Sy2 & 91 \\ 
NGC 3561 & 167.805000 &  28.696472 & 0.029367 & 14.7 & 13.8 & 13.1 & --22.5 & 1.36 & 0.51 & * &  8.4 & * & 0.0 & 0.44 & 0.0* & * & SB0-a & 4 & S0\string^0\string^: pec     Sy3 & 92 \\ 
IC 0676 & 168.165917 &   9.055833 & 0.004767 & 12.7 & 11.8 & 12.4 & --19.3 & 1.72 & 0.60 & * & 14.4 & 10.0 & 0.061 & 0.46 & --1.0 & 0.5 & SB0-a & 1 & (R)SB(r)0+     Sbrst & 93 \\ 
IC 2637 & 168.457292 &   9.586306 & 0.02923 & 13.9 & 12.9 & 12.9 & --22.7 & 0.92 & 0.87 & * &  3.6 & * & 0.017 & 0.42 & --4.0 & 0.9 & E0 & 4 & E+ pec         Sy1.5 & 94 \\ 
NGC 3593 & 168.654167 &  12.817667 & 0.002095 & 11.9 & 10.9 &  9.5 & --20.3 & 1.46 & 0.73 &  33.6 & 24.6 & 92.0 & 0.0 & 0.78 & -.0 & 0.4 & S0-a & 4 & SA(s)0/a;HII   Sy2 & 95 \\ 
NGC 3610 & 169.605292 &  58.786278 & 0.005694 & 11.7 & 10.8 & 10.4 & --21.7 & 1.83 & 0.89 &  15.3 &  6.0 & 144.0 & 0.0 & 0.45 & --5.0 & 0.4 & E5 & 0 & SB(r)0\string^0\string^ pec & 96 \\ 
NGC 3622 & 170.051542 &  67.241556 & 0.004325 & 13.7 & 13.2 & 13.2 & --18.2 & 1.31 & 0.55 &  11.4 &  7.8 & 7.0 & 0.0 & 0.10 & 3.0* & * & S? & 0 & S? & 97 \\ 
NGC 3640 & 170.278542 &   3.234833 & 0.00433 & 11.4 & 10.4 &  9.7 & --21.7 & 4.0 & 0.80 &  32.1 & 16.2 & 100.0 & 0.097 & 0.92 & --5.0 & 0.3 & E3 & 0 & E3 & 98 \\ 
NGC 3646 & 170.429500 &  20.169556 & 0.01417 & 11.8 & 11.1 & 10.4 & --23.6 & 3.9 & 0.56 &  54.6 & 36.6 & 50.0 & 0.0 & 0.15 & 4.0 & 0.3 & Sbc/P & 0 & SA:(r)bc pec (ring) & 99 \\ 
NGC 3655 & 170.727583 &  16.590028 & 0.004913 & 12.3 & 11.7 & 11.2 & --20.5 & 1.5 & 0.67 & * & 11.4 & 30.0 & 0.0 & 0.11 & 5.0 & 0.4 & Sc & 0 & SA(s)c:        HII & 100 \\ 
NGC 3656 & 170.911042 &  53.842111 & 0.00964 & 13.3 & 12.3 & 11.6 & --21.6 & 1.6 & 1.00 & * & 14.4 & * & 0.0 & 0.94 & 90.0 & * & E? & 3 & (R')I0: pec    LINER & 101 \\ 
NGC 3659 & 170.939750 &  17.818667 & 0.004287 & 12.8 & 12.2 & 12.8 & --18.6 & 2.1 & 0.52 & * & 10.8 & 60.0 & 0.0 & 0.06 & 9.0 & 0.8 & SBm & 0 & SB(s)m?        HII & 102 \\ 
NGC 3664 & 171.101042 &   3.325000 & 0.004607 & 15.1 & 14.5 &  7.7 & --23.9 & 2.0 & 0.95 &  35.1 & 19.2 & 15.0 & 0.109 & 0.01 & 9.0 & 0.4 & SBm & 0 & SB(s)m pec & 103 \\ 
IC 0692 & 171.472792 &   9.987500 & 0.003858 & 14.4 & 13.6 & 13.6 & --17.6 & 0.84 & 0.64 & * &  4.2 & 125.0 & 0.096 & 0.81 & --5.0 & * & S & 0 & E & 104 \\ 
IC 0691 & 171.684667 &  59.155417 & 0.003992 & 14.5 & 13.9 & 12.8 & --18.5 & 0.9 & 0.60 & * &  3.6 & 150.0 & 0.0 & 0.59 & 99.0 & * & P & 0 & I?;WR?         HII & 105 \\ 
NGC 3683 & 171.882708 &  56.877056 & 0.005724 & 13.2 & 12.5 & 10.7 & --21.3 & 1.84 & 0.53 & * &  8.4 & 128.0 & 0.0 & 0.30 & 5.0 & 0.9 & SBc & 0 & SB(s)c?        HII & 106 \\ 
NGC 3686 & 171.933208 &  17.224194 & 0.003856 & 11.9 & 11.3 & 10.6 & --20.6 & 3.2 & 0.78 &  37.8 & 33.0 & 15.0 & 0.023 & 0.05 & 4.0 & 0.5 & SBbc & 0 & SB(s)bc & 107 \\ 
NGC 3720 & 173.090000 &   0.804000 & 0.019837 & 13.7 & 13.0 & 12.6 & --22.2 & 1.0 & 0.90 &  11.1 &  6.6 & 85.0 & 0.077 & 0.12 & .9 & 0.7 & Sa & 0 & SAa: & 108 \\ 
NGC 3726 & 173.338000 &  47.029194 & 0.002887 & 10.9 & 10.4 & 10.0 & --20.6 & 6.2 & 0.69 & * & 61.2 & 10.0 & 0.008 & 0.03 & 5.0 & 0.3 & SBc & 0 & SAB(r)c        HII & 109 \\ 
NGC 3738 & 173.953292 &  54.523889 & 0.000764 & 12.1 & 11.7 & 12.2 & --15.5 & 2.5 & 0.76 & * & 24.0 & 155.0 & 0.0 & 0.11 & 10.0 & 0.3 & Im & 0 & Irr            HII & 110 \\ 
NGC 3741 & 174.025750 &  45.283639 & 0.000764 & 14.3 & 14.0 & 15.6 & --12.1 & 2.0 & 0.55 &  20.4 & 11.4 & 5.0 & 0.0 & 0.07 & 10.0 & 0.8 & Im & 0 & ImIII/BCD & 111 \\ 
NGC 3750 & 174.465167 &  21.974250 & 0.030291 & 14.9 & 13.9 & 13.4 & --22.3 & 0.8 & 0.87 & * &  6.6 & 132.0 & 0.0 & 0.88 & --3.0 & 0.7 & E-S0 & 0 & SAB0-? & 112 \\ 
NGC 3773 & 174.553667 &  12.112056 & 0.003276 & 13.0 & 12.0 & 13.1 & --17.7 & 1.2 & 0.83 & * &  9.0 & 165.0 & 0.089 & 0.52 & --2.0 & 0.6 & S0 & 0 & SA0:           HII & 113 \\ 
NGC 3781 & 174.765667 &  26.361750 & 0.022676 & 14.8 & 13.8 & 12.8 & --22.2 & 0.71 & 0.76 & * &  4.8 & 30.0 & 0.0 & 0.51 & 0.0* & * & S0 & 0 & S0/a & 114 \\ 
NGC 3794 & 175.222583 &  56.202028 & 0.00462 & 13.6 & 12.9 & 13.3 & --18.3 & 2.2 & 0.64 & * & 24.0 & 120.0 & 0.0 & 0.20 & 7.0* & * & SBc & 0 & SAB(s)d & 115 \\ 
NGC 3799 & 175.039083 &  15.327306 & 0.011048 & 14.7 & 13.9 & 13.6 & --19.8 & 0.8 & 0.62 & * &  6.0 & 114.0 & 0.055 & 0.02 & 3.0 & 0.5 & SBb/P & 0 & SB(s)b: pec & 116 \\ 
NGC 3801 & 175.070583 &  17.728056 & 0.011064 & 13.0 & 12.0 & 11.5 & --22.0 & 3.5 & 0.60 &  33.0 & 20.4 & 120.0 & 0.0 & 0.63 & --2.0 & 1.4 & S0 & 0 & S0/a & 117 \\ 
NGC 3811 & 175.319292 &  47.690806 & 0.010357 & 12.9 & 12.3 & 12.0 & --21.3 & 2.2 & 0.77 & * & 15.6 & 160.0 & 0.018 & 0.30 & 6.0 & 1.1 & SBc/P & 1 & SB(r)cd:       Sbrst & 118 \\ 
NGC 3822 & 175.546292 &  10.277778 & 0.020904 & 14.0 & 13.1 & 12.0 & --22.9 & 1.4 & 0.57 & * &  6.0 & 178.0 & 0.122 & 0.19 & --2.0 & 1.7 & S0 & 4 & Sb             Sy2 & 119 \\ 
NGC 3839 & 175.976375 &  10.784694 & 0.019734 & 13.9 & 13.3 & 12.9 & --21.9 & 1.14 & 0.53 & * &  6.6 & 87.0 & 0.195 & 0.25 & 8.0 & 1.3 & Sd & 0 & Sdm: & 120 \\ 
IC 0730 & 176.396875 &   3.231833 & 0.020198 & 14.6 & 13.7 & 12.8 & --22.0 & 0.91 & 0.62 & * &  3.6 & 36.0 & 0.049 & 0.62 & -.0 & 1.8 & S0-a & 0 & S0/a pec? & 121 \\ 
NGC 3870 & 176.485833 &  50.199750 & 0.002522 & 13.5 & 13.0 & 13.2 & --17.0 & 1.1 & 0.65 &   7.8 &  4.8 & 25.0 & 0.0 & 0.44 & --2.0 & 1.7 & S0 & 0 & S0? & 122 \\ 
NGC 3906 & 177.418750 &  48.425972 & 0.0032 & 13.8 & 12.9 & 12.9 & --17.9 & 1.9 & 0.89 & * & 22.2 & 0.0 & 0.027 & 0.04 & 7.0 & 0.8 & SBcd & 0 & SB(s)d & 123 \\ 
NGC 3921 & 177.778625 &  55.078750 & 0.019667 & 13.1 & 12.4 & 12.6 & --22.2 & 2.1 & 0.62 &  21.6 &  6.0 & 20.0 & 0.0 & 0.26 & -.0 & 0.4 & S0-a & 0 & (R')SA(s)0/a pec & 124 \\ 
NGC 3928 & 177.948417 &  48.683139 & 0.003296 & 13.2 & 12.6 & 12.0 & --18.8 & 1.29 & 0.92 &  11.4 &  6.0 & * & 0.038 & 0.89 & 3.0* & * & E0 & 0 & SA(s)b?        HII & 125 \\ 
NGC 3934 & 178.052333 &  16.851444 & 0.012605 & 14.4 & 13.6 & 12.8 & --20.9 & 1.1 & 0.91 & * & 10.8 & 66.0 & 0.135 & 0.68 & 0.0* & * & Sb & 0 & S0/a & 126 \\ 
NGC 3938 & 178.206042 &  44.120722 & 0.002699 & 10.9 & 10.4 & 10.2 & --20.2 & 5.4 & 0.91 &  72.0 & 54.6 & 0.0 & 0.0 & 0.16 & 5.0 & 0.3 & Sc & 0 & SA(s)c         HII & 127 \\ 
NGC 3941 & 178.230667 &  36.986333 & 0.003102 & 11.3 & 10.3 &  9.9 & --20.8 & 3.5 & 0.66 &  22.8 & 11.4 & 10.0 & 0.0 & 0.49 & --2.0 & 0.3 & SB0 & 4 & SB(s)0\string^0\string^      Sy2 & 128 \\ 
NGC 3945 & 178.307208 &  60.675556 & 0.004273 & 11.8 & 10.9 &  9.7 & --21.7 & 5.2 & 0.67 &  22.8 & 10.2 & 160.0 & 0.073 & 0.58 & --1.0 & 0.3 & SB0 & 3 & SB(rs)0+       LINER & 129 \\ 
NGC 4014 & 179.649208 &  16.177306 & 0.012552 & 13.2 & 12.3 & 11.3 & --22.4 & 2.2 & 0.59 & * &  6.6 & 120.0 & 0.088 & 0.64 & -.0 & 0.8 & S0-a & 0 & S0/a & 130 \\ 
NGC 4068 & 181.003250 &  52.588278 & 0.0007 & 13.0 & 12.4 & 11.0 & --16.4 & 3.3 & 0.52 & * &  1.8 & 30.0 & 0.0 & 0.09 & 10.0 & 0.5 & Im & 0 & IAm & 131 \\ 
NGC 4073 & 181.112792 &   1.895972 & 0.019584 & 12.4 & 11.4 & 10.8 & --23.9 & 1.93 & 0.63 &  47.4 & 24.0 & 105.0 & 0.008 & 0.85 & --3.8 & 0.4 & E3 & 0 & E;BrClG & 132 \\ 
NGC 4125 & 182.025083 &  65.174139 & 0.004523 & 10.7 & 9.7 &  9.1 & --22.4 & 5.8 & 0.55 &  58.5 & 21.6 & 81.0 & 0.037 & 0.82 & --5.0 & 0.3 & E6/P & 3 & E6 pec         LINER & 133 \\ 
NGC 4136 & 182.323708 &  29.927611 & 0.002031 & 11.8 & 11.1 & 11.8 & --17.9 & 4.0 & 0.93 & * & 40.2 & 90.0 & 0.022 & 0.03 & 5.0 & 0.5 & SBc & 0 & SAB(r)c        HII & 134 \\ 
NGC 4150 & 182.640208 &  30.401528 & 0.000694 & 12.4 & 11.6 & 11.4 & --16.0 & 2.3 & 0.70 &  17.7 &  9.0 & 147.0 & 0.044 & 0.21 & --2.0 & 0.4 & S0 & 0 & SA(r)0\string^0\string^? & 135 \\ 
NGC 4162 & 182.968625 &  24.123667 & 0.008569 & 12.9 & 12.2 & 11.8 & --21.1 & 2.3 & 0.61 &  21.3 & 17.4 & 174.0 & 0.089 & 0.07 & 4.0 & 0.4 & Sbc & 5 & (R)SA(rs)bc    AGN & 136 \\ 
NGC 4168 & 183.071958 &  13.205194 & 0.007625 & 12.1 & 11.2 & 10.7 & --22.0 & 2.03 & 0.78 &  28.5 & 21.0 & 120.0 & 0.026 & 0.90 & --5.0 & 0.3 & E2 & 4 & E2             Sy1.9 & 137 \\ 
IC 3050 & 183.446958 &  13.424806 & 0.007055 & 12.5 & 11.7 & 10.6 & --21.9 & 2.4 & 0.71 & * & 29.4 & 85.0 & 0.025 & 0.02 & 5.0* & * & SBc & 0 & SAB(rs)cd?     HII & 138 \\ 
NGC 4194 & 183.539458 &  54.526833 & 0.008342 & 13.0 & 12.5 & 12.0 & --20.9 & 1.8 & 0.61 &   7.5 &  3.0 & 168.0 & 0.0 & 0.79 & 10.0 & 0.4 & IBm/P & 0 & IBm pec;BlueCG HII & 139 \\ 
NGC 4207 & 183.877083 &   9.584889 & 0.001988 & 13.6 & 12.6 & 11.9 & --17.8 & 1.59 & 0.57 & * & 12.6 & 124.0 & 0.0 & 0.25 & 6.0* & * & Scd & 0 & Scd            HII & 140 \\ 
NGC 4234 & 184.288167 &   3.683056 & 0.006761 & 13.3 & 12.7 & 12.2 & --20.2 & 1.37 & 0.77 & * & 16.2 & * & 0.014 & 0.18 & 8.7 & 0.5 & SBm & 0 & (R')SB(s)m     HII & 141 \\ 
NGC 4267 & 184.938500 &  12.798278 & 0.003406 & 11.9 & 10.9 &  9.8 & --21.1 & 3.2 & 0.94 &  41.4 & 18.6 & 33.0 & 0.024 & 0.30 & --3.0 & 0.3 & E/SB0 & 0 & SB(s)0-? & 142 \\ 
NGC 4290 & 185.198042 &  58.092500 & 0.010114 & 12.8 & 12.0 & 11.8 & --21.5 & 2.02 & 0.62 & * & 19.8 & 90.0 & 0.0 & 0.21 & 2.0 & 0.5 & SBab & 0 & SB(rs)ab:      HII & 143 \\ 
NGC 4335 & 185.757833 &  58.444556 & 0.015417 & 13.4 & 12.4 & 11.6 & --22.6 & 1.9 & 0.79 & * &  9.0 & 145.0 & 0.0 & 0.64 & --5.0 & 0.8 & E2 & 0 & E & 144 \\ 
NGC 4365 & 186.117833 &   7.317667 & 0.004146 & 10.5 & 9.6 &  8.8 & --22.6 & 6.9 & 0.72 &  49.8 & 42.0 & 40.0 & 0.0 & 0.67 & --5.0 & 0.3 & E3 & 0 & E3 & 145 \\ 
NGC 4369 & 186.150833 &  39.383000 & 0.003486 & 12.3 & 11.7 & 10.8 & --20.2 & 2.1 & 0.95 &  16.5 & 13.2 & 127.0 & 0.0 & 0.90 & 1.0 & 0.3 & Sa & 0 & (R)SA(rs)a     HII & 146 \\ 
NGC 4378 & 186.325417 &   4.925139 & 0.008536 & 12.6 & 11.7 & 11.2 & --21.7 & 2.9 & 0.93 &  18.6 & 13.2 & 167.0 & 0.0 & 0.47 & 1.0 & 0.3 & Sa & 4 & (R)SA(s)a      Sy2 & 147 \\ 
NGC 4414 & 186.612917 &  31.223528 & 0.002388 & 11.0 & 10.1 &  9.4 & --20.7 & 3.6 & 0.56 &  27.3 & 21.0 & 155.0 & 0.019 & 0.07 & 5.0 & 0.3 & Sc & 3 & SA(rs)c?;HII   LINER & 148 \\ 
NGC 4412 & 186.650333 &   3.964694 & 0.007652 & 13.2 & 12.4 & 12.2 & --20.5 & 1.4 & 0.93 & * & 17.4 & 132.0 & 0.028 & 0.08 & 3.0 & 0.4 & SBb/P & 3 & SB(r)b? pec    LINER & 149 \\ 
NGC 4420 & 186.743750 &   2.494361 & 0.005621 & 12.8 & 12.1 & 11.5 & --20.5 & 1.44 & 0.60 & * & 12.6 & 8.0 & 0.0 & 0.14 & 4.0 & 0.6 & SBbc & 3 & SB(r)bc:;HII   LINER & 150 \\ 
NGC 4449 & 187.046250 &  44.093639 & 0.00069 & 10.0 & 9.6 &  9.9 & --17.5 & 6.2 & 0.71 &  48.6 & 43.2 & 45.0 & 0.0 & 0.11 & 10.0 & 0.3 & IBm & 1 & IBm;HII        Sbrst & 151 \\ 
NGC 4450 & 187.123458 &  17.084944 & 0.006518 & 10.9 & 10.1 &  9.7 & --22.7 & 5.2 & 0.75 &  61.2 & 42.0 & 175.0 & 0.025 & 0.27 & 2.0 & 0.3 & Sab & 3 & SA(s)ab;LINER  Sy3 & 152 \\ 
NGC 4457 & 187.245875 &   3.570583 & 0.002942 & 11.8 & 10.9 & 10.2 & --20.3 & 2.7 & 0.85 &  17.4 & 10.8 & 66.0 & 0.035 & 0.57 & -.0 & 0.3 & SB0-a & 3 & (R)SAB(s)0/a   LINER & 153 \\ 
NGC 4494 & 187.850417 &  25.775250 & 0.004476 & 10.7 & 9.8 &  9.3 & --22.2 & 4.8 & 0.73 &  48.6 & 25.8 & 171.0 & 0.051 & 0.97 & --5.0 & 0.3 & E1 & 3 & E1-2           LINER & 154 \\ 
NGC 4500 & 187.842333 &  57.964639 & 0.010377 & 13.1 & 12.5 & 12.2 & --21.1 & 1.6 & 0.62 & * &  5.4 & 130.0 & 0.0 & 0.33 & 1.0 & 0.4 & SBa & 1 & SB(s)a         Sbrst & 155 \\ 
NGC 4498 & 187.914833 &  16.852778 & 0.005027 & 12.8 & 12.1 & 12.1 & --19.7 & 3.0 & 0.53 & * & 25.8 & 133.0 & 0.026 & 0.17 & 6.5 & 0.5 & SBc & 0 & SAB(s)d        HII & 156 \\ 
NGC 4509 & 188.278292 &  32.091556 & 0.003125 & 14.3 & 13.5 & 14.6 & --16.1 & 0.9 & 0.67 & * &  7.2 & 155.0 & 0.02 & 0.01 & 2.0 & 0.9 & Sab/P & 0 & Sab pec?       HII & 157 \\ 
IC 0800 & 188.486083 &  15.354833 & 0.007759 & 14.1 & 13.4 & 13.0 & --19.7 & 1.51 & 0.67 & * & 20.4 & 157.0 & 0.043 & 0.17 & 4.7 & 0.9 & SBc & 0 & SB(rs)c pec?   HII & 158 \\ 
NGC 4561 & 189.034167 &  19.322917 & 0.004677 & 12.9 & 12.5 & 12.8 & --18.8 & 1.5 & 0.87 &  28.5 & 18.0 & 30.0 & -- & 0.16 & 8.0 & 0.4 & SBcd & 0 & SB(rs)dm & 159 \\ 
NGC 4578 & 189.377333 &   9.555083 & 0.007645 & 12.4 & 11.5 & 10.6 & --22.1 & 3.3 & 0.76 &  32.1 & 21.6 & 35.0 & 0.0 & 0.44 & --2.0 & 0.5 & S0 & 0 & SA(r)0\string^0\string^: & 160 \\ 
NGC 4580 & 189.451625 &   5.368528 & 0.003449 & 12.3 & 11.8 & 11.3 & --19.6 & 2.28 & 0.64 &  27.3 & 24.0 & 165.0 & 0.0 & 0.01 & 1.0 & 0.3 & SBa/P & 3 & SAB(rs)a pec   LINER & 161 \\ 
NGC 4612 & 190.386458 &   7.314889 & 0.005921 & 12.5 & 11.5 & 11.3 & --20.8 & 2.17 & 0.64 & * & 13.2 & 145.0 & 0.009 & 0.30 & --2.0 & 0.4 & SB0 & 0 & (R)SAB0\string^0\string^ & 162 \\ 
IC 3687 & 190.562917 &  38.503333 & 0.001181 & 13.7 & 13.5 & 15.5 & --13.1 & 3.4 & 0.88 &  41.4 & 23.4 & 9.0 & 0.0 & 0.00 & 10.0 & 0.5 & IBm & 0 & IAB(s)m & 163 \\ 
NGC 4636 & 190.707625 &   2.687778 & 0.003129 & 10.4 & 9.5 &  8.9 & --21.8 & 6.0 & 0.78 &  88.5 & 58.2 & 150.0 & 0.05 & 0.76 & --5.0 & 0.3 & E2 & 3 & E/S0\_1;LINER   Sy3 & 164 \\ 
NGC 4651 & 190.927625 &  16.393389 & 0.002628 & 11.4 & 10.8 & 10.5 & --19.8 & 4.0 & 0.65 &  36.0 & 21.6 & 80.0 & 0.028 & 0.06 & 5.0 & 0.3 & Sc/P & 3 & SA(rs)c        LINER & 165 \\ 
NGC 4670 & 191.321125 &  27.125417 & 0.003566 & 13.1 & 12.7 & 12.9 & --18.1 & 1.4 & 0.79 & * &  6.0 & 90.0 & 0.043 & 0.31 & -.0 & 0.4 & SB0-a & 0 & SB(s)0/a pec:  BCDG & 166 \\ 
NGC 4688 & 191.943833 &   4.336056 & 0.003289 & 12.6 & 11.9 & 13.2 & --17.6 & 3.2 & 0.87 & * & 24.6 & 123.0 & 0.013 & 0.34 & 6.0 & 0.5 & SBc & 3 & SB(s)cd;LINER  HII & 167 \\ 
NGC 4689 & 191.939833 &  13.762806 & 0.00539 & 11.6 & 11.0 & 10.5 & --21.4 & 4.3 & 0.81 & * & 48.0 & 160.0 & 0.048 & 0.11 & 4.0 & 0.3 & Sbc & 3 & SA(rs)bc;Sy    LINER & 168 \\ 
NGC 4698 & 192.095458 &   8.487389 & 0.003366 & 11.5 & 10.6 & 10.2 & --20.7 & 4.0 & 0.62 &  33.0 & 18.6 & 170.0 & 0.0 & 0.33 & 2.0 & 0.3 & Sab & 3 & SA(s)ab;Sy2    LINER & 169 \\ 
NGC 4704 & 192.193458 &  41.921250 & 0.027132 & 14.5 & 13.7 & 12.7 & --22.8 & 1.0 & 0.90 &  12.3 & 12.0 & 105.0 & 0.0 & 0.15 & 3.5 & 0.6 & SBbc/P & 4 & Sbc pec;HII    Sy2 & 170 \\ 
NGC 4701 & 192.298292 &   3.388722 & 0.002406 & 12.8 & 12.4 & 12.4 & --17.8 & 2.8 & 0.75 & * & 12.0 & 45.0 & 0.014 & 0.46 & 6.0 & 0.3 & Sc & 0 & SA(s)cd        HII & 171 \\ 
NGC 4713 & 192.491125 &   5.311417 & 0.002183 & 12.2 & 11.7 & 11.7 & --18.2 & 2.28 & 0.68 &  32.1 & 25.8 & 100.0 & 0.0 & 0.01 & 7.0 & 0.3 & SBcd & 3 & SAB(rs)d;HII   LINER & 172 \\ 
NGC 4736 & 192.721083 &  41.120444 & 0.001027 & 9.0 & 8.2 &  7.6 & --20.7 & 11.2 & 0.81 &  38.7 & 19.2 & 117.0 & 0.0 & 0.82 & 2.0 & 0.3 & Sab & 3 & (R)SA(r)ab;Sy2 LINER & 173 \\ 
NGC 4765 & 193.310042 &   4.463111 & 0.002388 & 13.4 & 13.0 & 13.4 & --16.7 & 1.1 & 0.73 &   7.8 &  6.0 & 80.0 & 0.006 & 0.04 & -.0 & 1.7 & S0-a & 0 & S0/a?          HII & 174 \\ 
NGC 4772 & 193.371500 &   2.168389 & 0.003469 & 12.0 & 11.0 & 10.9 & --20.0 & 3.4 & 0.50 &  23.7 & 21.0 & 147.0 & 0.0 & 0.51 & 1.0 & 0.3 & Sa & 3 & SA(s)a;LINER   Sy3 & 175 \\ 
NGC 4868 & 194.787083 &  37.310333 & 0.015561 & 13.0 & 12.2 & 11.8 & --22.4 & 1.6 & 0.94 & * & 13.2 & 90.0 & 0.0 & 0.07 & 2.3 & 0.6 & Sab & 0 & SAab? & 176 \\ 
IC 4182 & 196.456417 &  37.604889 & 0.001071 & 11.8 & 11.1 & 14.1 & --14.3 & 6.0 & 0.92 & * & 91.8 & 90.0 & 0.0 & 0.00 & 9.0 & 0.4 & Sm & 0 & SA(s)m & 177 \\ 
NGC 4992 & 197.273333 &  11.634167 & 0.025137 & 14.3 & 13.4 & 12.8 & --22.5 & 1.18 & 0.58 & * &  7.2 & 10.0 & 0.016 & 0.22 & 1.0 & 0.9 & Sa & 4 & Sa;XBONG       Sy2 & 178 \\ 
NGC 5060 & 199.317583 &   6.037444 & 0.020791 & 14.1 & 13.3 & 12.2 & --22.7 & 1.1 & 0.73 & * & 12.0 & 55.0 & 0.0 & 0.29 & 3.0 & 0.9 & SBb & 0 & SB(s)b & 179 \\ 
NGC 5068 & 199.728375 & --21.039111 & 0.002235 & 10.7 & 10.0 &  9.8 & --20.2 & 7.2 & 0.88 &  73.5 & 84.0 & 110.0 & 0.309 & 0.28 & 6.0 & 0.3 & SBc & 0 & SB(s)d & 180 \\ 
NGC 5123 & 200.793833 &  43.086250 & 0.027546 & 13.5 & 12.8 & 12.5 & --22.9 & 1.2 & 0.93 & * & 12.6 & 174.0 & 0.0 & 0.16 & 6.0 & 1.2 & Sc & 0 & Scd: & 181 \\ 
NGC 5127 & 200.937583 &  31.565750 & 0.016218 & 12.9 & 11.9 & 12.1 & --22.3 & 1.54 & 0.70 & * & 13.2 & 75.0 & 0.023 & 0.52 & --5.0 & 0.5 & E2 & 0 & E pec & 182 \\ 
NGC 5141 & 201.214333 &  36.378528 & 0.017379 & 13.8 & 12.8 & 12.3 & --22.1 & 1.3 & 0.77 & * &  4.2 & 80.0 & 0.0 & 0.60 & --2.0 & 0.8 & S0 & 0 & S0 & 183 \\ 
NGC 5147 & 201.582208 &   2.100861 & 0.003629 & 12.3 & 11.8 & 10.9 & --20.2 & 1.9 & 0.79 &  21.3 & 21.0 & 120.0 & 0.0 & 0.15 & 8.0 & 0.4 & SBd & 0 & SB(s)dm        HII & 184 \\ 
NGC 5198 & 202.547500 &  46.670778 & 0.008402 & 12.7 & 11.8 & 11.5 & --21.4 & 2.1 & 0.86 &  25.5 & 10.8 & 0.0 & 0.0 & 0.42 & --5.0 & 0.5 & E1 & 0 & E1-2: & 185 \\ 
NGC 5230 & 203.882833 &  13.676167 & 0.022856 & 12.8 & 12.1 & 12.1 & --22.9 & 2.2 & 0.86 & * & 22.8 & * & 0.0 & 0.09 & 5.0 & 0.3 & SBc & 0 & SA(s)c         HII & 186 \\ 
NGC 5248 & 204.383417 &   8.885167 & 0.003839 & 11.0 & 10.3 &  9.7 & --21.5 & 6.2 & 0.73 &  53.4 & 35.4 & 122.0 & 0.0 & 0.48 & 4.0 & 0.3 & SBbc & 4 & (R)SB(rs)bc;Sy2HII & 187 \\ 
NGC 5257 & 204.970458 &   0.840000 & 0.022676 & 12.9 & 12.4 & 12.3 & --22.7 & 1.8 & 0.50 & * &  9.6 & 121.0 & 0.009 & 0.27 & 3.0 & 0.4 & SBb/P & 2 & SAB(s)b pec;HIILIRG & 188 \\ 
NGC 5258 & 204.990375 &   0.830944 & 0.022539 & 12.9 & 12.3 & 11.6 & --23.4 & 1.7 & 0.65 & * &  9.0 & 22.0 & 0.009 & 0.27 & 3.0 & 0.4 & SBb & 3 & SA(s)b: pec;HIILINER & 189 \\ 
NGC 5278 & 205.415083 &  55.670639 & 0.025154 & 13.7 & 12.9 & 10.9 & --24.3 & 1.3 & 0.77 & * &  9.0 & 57.0 & 0.0 & 0.28 & 3.0 & 0.4 & Sb/P & 0 & SA(s)b? pec & 190 \\ 
NGC 5273 & 205.534750 &  35.654222 & 0.003619 & 12.4 & 11.6 & 11.1 & --19.9 & 1.94 & 0.93 &  30.6 & 23.4 & 10.0 & 0.0 & 0.17 & --2.0 & 0.3 & S0 & 4 & SA(s)0\string^0\string^      Sy1.9 & 191 \\ 
NGC 5313 & 207.434750 &  39.984778 & 0.008466 & 12.8 & 12.0 & 10.9 & --22.0 & 1.41 & 0.67 & * & 12.6 & 43.0 & 0.0 & 0.08 & 3.0 & 1.6 & Sb & 0 & Sb? & 192 \\ 
NGC 5368 & 208.621500 &  54.330667 & 0.015531 & 13.8 & 13.0 & 12.5 & --21.7 & 1.16 & 0.67 & * &  6.0 & 10.0 & 0.0 & 0.54 & 1.5 & 0.6 & SBab & 0 & (R')SABab: & 193 \\ 
NGC 5363 & 209.030042 &   5.254778 & 0.003799 & 11.1 & 10.1 &  9.5 & --21.6 & 4.1 & 0.63 &  36.0 & 27.0 & 135.0 & 0.038 & 0.82 & 90.0 & * & S0-a & 3 & I0?            LINER & 194 \\ 
NGC 5374 & 209.373458 &   6.097000 & 0.014617 & 13.3 & 12.5 & 11.8 & --22.3 & 1.7 & 0.88 & * & 16.8 & 54.0 & 0.023 & 0.13 & 3.7 & 0.6 & SBbc & 0 & SB(r)bc? & 195 \\ 
NGC 5414 & 210.514708 &   9.929333 & 0.014206 & 13.4 & 12.4 & 12.7 & --21.3 & 1.0 & 0.80 & * &  4.8 & 172.0 & 0.006 & 0.28 & 99.0 & * & P & 0 & PECULR & 196 \\ 
NGC 5448 & 210.708458 &  49.172694 & 0.006748 & 11.9 & 11.0 & 11.2 & --21.1 & 1.49 & 0.68 &  72.0 & 15.6 & 115.0 & 0.041 & 0.20 & 1.0 & 0.3 & SBa & 5 & (R)SAB(r)a     AGN & 197 \\ 
NGC 5490 & 212.488708 &  17.545556 & 0.016195 & 13.1 & 12.1 & 11.5 & --22.8 & 1.74 & 0.64 &  18.6 &  6.0 & 5.0 & 0.0 & 0.75 & --5.0 & 0.5 & E2 & 0 & E & 198 \\ 
NGC 5520 & 213.094958 &  50.348417 & 0.006261 & 13.2 & 12.4 & 11.3 & --20.9 & 2.0 & 0.55 & * &  7.8 & 66.0 & 0.0 & 0.47 & 3.0 & 0.8 & Sb & 0 & Sb & 199 \\ 
NGC 5515 & 213.159042 &  39.310278 & 0.025749 & 13.7 & 12.9 & 12.4 & --22.9 & 1.31 & 0.53 & * &  4.8 & 108.0 & 0.0 & 0.27 & 2.0 & 0.8 & Sab & 4 & Sab            Sy1.9 & 200 \\ 
NGC 5541 & 214.132500 &  39.589056 & 0.025678 & 13.6 & 12.7 & 12.3 & --23.0 & 0.95 & 0.69 & * &  7.2 & 12.0 & 0.0 & 0.07 & 5.0* & * & S? & 0 & Sc             HII & 201 \\ 
NGC 5532 & 214.220625 &  10.807389 & 0.024704 & 12.9 & 11.9 & 11.2 & --24.0 & 1.32 & 0.77 &  23.4 & 12.6 & * & 0.0 & 0.79 & --2.0 & 0.8 & S0 & 0 & FRI            LEG & 202 \\ 
NGC 5557 & 214.607167 &  36.493556 & 0.010737 & 11.9 & 11.0 & 10.6 & --22.8 & 1.93 & 0.82 &  30.0 & 13.8 & 105.0 & 0.0 & 0.61 & --5.0 & 0.3 & E1 & 0 & E1 & 203 \\ 
NGC 5585 & 214.950833 &  56.729056 & 0.000977 & 11.2 & 10.7 &  9.3 & --18.8 & 5.8 & 0.64 & 101.7 & 45.6 & 30.0 & 0.0 & 0.39 & 7.0 & 0.3 & SBcd & 0 & SAB(s)d        HII & 204 \\ 
NGC 5576 & 215.265333 &   3.271000 & 0.005023 & 11.9 & 11.0 & 10.3 & --21.5 & 3.5 & 0.63 &  18.0 &  7.8 & 95.0 & 0.037 & 0.73 & --5.0 & 0.3 & E3 & 0 & E3 & 205 \\ 
NGC 5584 & 215.599042 & --0.387667 & 0.005464 & 12.1 & 11.4 & 11.4 & --20.5 & 2.45 & 0.67 & * & 39.6 & 140.0 & 0.145 & 0.03 & 6.0 & 0.3 & SBc & 0 & SAB(rs)cd & 206 \\ 
NGC 5596 & 215.619750 &  37.122194 & 0.010414 & 14.4 & 13.5 & 12.9 & --20.5 & 1.13 & 0.65 &   9.6 &  6.0 & 100.0 & 0.0 & 0.41 & --2.0 & 0.8 & S0 & 0 & S0 & 207 \\ 
NGC 5631 & 216.638750 &  56.582639 & 0.006484 & 12.4 & 11.5 & 11.0 & --21.3 & 1.86 & 0.87 &  18.9 & 12.0 & * & 0.0 & 0.56 & --2.0 & 0.3 & S0 & 4 & SA(s)0\string^0\string^      Sy2 & 208 \\ 
NGC 5633 & 216.868250 &  46.146528 & 0.007785 & 13.1 & 12.4 & 11.9 & --20.8 & 1.56 & 0.62 &  15.6 & 10.2 & 10.0 & 0.039 & 0.01 & 3.0 & 0.4 & Sb & 0 & (R)SA(rs)b & 209 \\ 
NGC 5660 & 217.457542 &  49.622667 & 0.007765 & 12.4 & 11.9 & 11.8 & --20.9 & 2.8 & 0.89 &  25.5 & 24.0 & 90.0 & 0.0 & 0.30 & 5.0 & 0.3 & SBc & 0 & SAB(rs)c & 210 \\ 
NGC 5653 & 217.543417 &  31.215500 & 0.011881 & 12.9 & 12.2 & 11.4 & --22.2 & 1.7 & 0.76 & * &  8.4 & 125.0 & 0.0 & 0.35 & 3.0 & 0.4 & Sb & 2 & (R')SA(rs)b;HIILIRG & 211 \\ 
NGC 5669 & 218.181208 &   9.890444 & 0.004563 & 12.0 & 11.3 & 12.5 & --19.1 & 4.0 & 0.70 & * & 40.8 & 50.0 & 0.021 & 0.03 & 6.0 & 0.3 & SBc & 0 & SAB(rs)cd & 212 \\ 
NGC 5668 & 218.351417 &   4.450444 & 0.00526 & 12.2 & 11.5 & 11.9 & --20.0 & 3.3 & 0.91 &  37.8 & 32.4 & * & 0.053 & 0.40 & 7.0 & 0.3 & Sd & 0 & SA(s)d & 213 \\ 
NGC 5691 & 219.472250 & --0.398889 & 0.006238 & 12.3 & 11.8 & 12.4 & --19.9 & 1.9 & 0.74 &  19.8 & 13.2 & 110.0 & 0.121 & 0.10 & 1.0 & 0.4 & SBa/P & 0 & SAB(s)a: pec   HII & 214 \\ 
IC 1065 & 222.339875 &  63.270556 & 0.041639 & 14.4 & 13.6 & 13.2 & --23.2 & 0.8 & 0.95 &  11.4 &  5.4 & 141.0 & 0.029 & 0.51 & --2.0 & 0.8 & SB0 & 0 & SB0;Radio galaxy & 215 \\ 
NGC 5778 & 223.631208 &  18.642306 & 0.055502 & 14.8 & 13.8 & 13.3 & --23.7 & 1.2 & 0.75 & * & 11.4 & 10.0 & 0.025 & 0.47 & --5.0 & 1.7 & E3 & 0 & cD;BrClG & 216 \\ 
IC 1076 & 223.748417 &  18.037333 & 0.020247 & 14.2 & 13.7 & 13.0 & --21.8 & 1.0 & 0.50 & * &  5.4 & 5.0 & 0.025 & 0.33 & 4.0* & * & Sbc & 1 & SBc            Sbrst & 217 \\ 
NGC 5820 & 224.665917 &  53.886083 & 0.011124 & 13.4 & 12.5 & 11.7 & --21.8 & 1.7 & 0.65 & * &  5.4 & 87.0 & 0.025 & 0.69 & --2.0 & 0.3 & S0 & 0 & S0 & 218 \\ 
NGC 5813 & 225.296792 &   1.701972 & 0.006525 & 11.5 & 10.5 & 10.1 & --22.2 & 4.2 & 0.71 &  57.3 & 31.8 & 145.0 & 0.149 & 0.41 & --5.0 & 0.3 & E1 & 3 & E1-2           LINER & 219 \\ 
NGC 5831 & 226.029167 &   1.219917 & 0.005524 & 12.5 & 11.5 & 10.9 & --21.0 & 1.94 & 0.82 &  25.5 & 14.4 & 55.0 & 0.137 & 0.58 & --5.0 & 0.4 & E3 & 5 & E3             BLLAC & 220 \\ 
NGC 5936 & 232.503458 &  12.989333 & 0.013356 & 13.1 & 12.5 & 11.7 & --22.2 & 1.4 & 0.93 & * & 14.4 & 36.0 & 0.093 & 0.20 & 3.0 & 0.4 & SBb & 2 & SB(rs)b;LIRG   HII & 221 \\ 
NGC 5953 & 233.634917 &  15.193778 & 0.006555 & 13.2 & 12.3 & 10.7 & --21.6 & 1.35 & 0.86 & * &  4.8 & 169.0 & 0.093 & 0.53 & 1.0 & 0.4 & S0-a & 4 & SAa: pec;LINER;Sy2 & 222 \\ 
NGC 5964 & 234.400917 &   5.974028 & 0.004827 & 12.6 & 11.9 & 11.5 & --20.1 & 4.2 & 0.76 & * & 52.8 & 145.0 & 0.145 & 0.24 & 7.0 & 0.3 & SBcd & 3 & SB(rs)d        AGN? & 223 \\ 
NGC 5982 & 234.665958 &  59.355833 & 0.010064 & 12.0 & 11.1 & 10.5 & --22.7 & 2.26 & 0.62 &  23.7 & 11.4 & 110.0 & 0.013 & 0.87 & --5.0 & 0.3 & E3 & 3 & E3             LINER & 224 \\ 
NGC 5992 & 236.089625 &  41.086361 & 0.031749 & 14.3 & 13.7 & 13.3 & --22.5 & 0.9 & 0.78 & * &  4.2 & 175.0 & 0.053 & 0.60 & 2.0* & * & Sab & 0 & SBb            HII & 225 \\ 
NGC 5990 & 236.568167 &   2.415417 & 0.012806 & 13.3 & 12.4 & 11.0 & --22.8 & 1.5 & 0.60 & * &  9.0 & 115.0 & 0.293 & 0.42 & 1.0 & 1.2 & Sa & 4 & (R')Sa pec?;Sy2LIRG & 226 \\ 
IC 1144 & 237.840375 &  43.417667 & 0.040291 & 14.5 & 13.5 & 13.3 & --23.1 & 0.7 & 0.86 & * &  3.0 & 100.0 & 0.033 & 0.54 & --3.0 & 1.3 & E-S0 & 0 & S0-: & 227 \\ 
NGC 6047 & 241.287458 &  17.729889 & 0.031262 & 14.6 & 13.5 & 13.0 & --22.8 & 1.1 & 0.73 &  17.7 &  9.6 & 90.0 & 0.061 & 0.65 & --4.0 & 0.5 & E3 & 0 & E+ & 228 \\ 
NGC 6109 & 244.418833 &  35.004278 & 0.029544 & 13.8 & 12.7 & 12.8 & --22.9 & 1.06 & 0.94 &  25.5 &  6.0 & * & 0.013 & 0.60 & --2.0 & * & S0 & 3 & E/S0;BrClG;LERGLINER & 229 \\ 
NGC 6137 & 245.762917 &  37.922361 & 0.031031 & 13.4 & 12.4 & 11.6 & --24.1 & 1.9 & 0.63 &  25.5 &  9.0 & 175.0 & 0.005 & 0.88 & --5.0 & 0.8 & E4 & 0 & E & 230 \\ 
NGC 6166 & 247.160333 &  39.551556 & 0.030354 & 12.8 & 11.8 & 10.9 & --24.8 & 1.9 & 0.74 &  47.4 & 16.2 & 35.0 & 0.0 & 0.89 & --4.0 & 0.4 & E3 & 0 & cD;E;NLRG      LEG & 231 \\ 
NGC 6240 & 253.245292 &   2.400917 & 0.02448 & 13.8 & 12.9 & 11.3 & --23.9 & 2.1 & 0.52 & * & 12.0 & 20.0 & 0.285 & 0.48 & 90.0 & * & E? & 3 & I0: pec;LINER  Sy2 & 232 \\ 
NGC 6340 & 257.603542 &  72.304444 & 0.003996 & 11.9 & 11.0 & 10.6 & --20.7 & 3.2 & 0.94 &  42.3 & 25.2 & 120.0 & 0.197 & 0.26 & -.0 & 0.3 & S0-a & 3 & SA(s)0/a       LINER & 233 \\ 
NGC 6338 & 258.845792 &  57.411194 & 0.027303 & 13.4 & 12.3 & 11.8 & --23.7 & 1.56 & 0.64 &  28.5 & 12.6 & 15.0 & 0.073 & 0.58 & --2.0 & 0.8 & S0 & 5 & cD;S0;PEG     blazar & 234 \\ 
IC 1262 & 263.258417 &  43.759611 & 0.032649 & 14.7 & 13.6 & 12.9 & --23.0 & 1.2 & 0.50 &  12.3 &  7.8 & 85.0 & 0.069 & 0.75 & --5.0 & 0.8 & E5 & 0 & cD;E & 235 \\ 
NGC 6789 & 289.175667 &  63.971472 & -0.00047 & 13.8 & 13.2 & 14.0 & --13.8 & 1.3 & 0.77 & * & 16.8 & 60.0 & 0.325 & 0.00 & 10.0 & 0.8 & Im & 0 & Im & 236 \\ 
NGC 7047 & 319.115208 & --0.826500 & 0.019383 & 14.2 & 13.4 & 12.4 & --22.3 & 1.38 & 0.50 & * & 12.0 & 107.0 & 0.149 & 0.02 & 3.0 & 1.2 & SBb & 0 & SAB(r)b:       HII & 237 \\ 
NGC 7077 & 322.498375 &   2.414167 & 0.003843 & 14.1 & 13.1 & 13.9 & --17.2 & 0.8 & 0.87 & * &  5.4 & 37.0 & 0.165 & 0.47 & --3.5 & 1.3 & E1 & 0 & BCD/E          HII & 238 \\ 
NGC 7080 & 322.508125 &  26.717806 & 0.016141 & 13.1 & 12.3 & 11.6 & --22.7 & 1.8 & 0.94 &  36.0 & 18.0 & 50.0 & 0.425 & 0.23 & 3.0 & 0.8 & SBb & 0 & SB(r)b & 239 \\ 
NGC 7177 & 330.171833 &  17.738056 & 0.003803 & 12.0 & 11.2 & 10.7 & --20.4 & 3.1 & 0.65 &  22.2 & 11.4 & 93.0 & 0.233 & 0.48 & 3.0 & 0.3 & SBb & 3 & SAB(r)b; HII   LINER & 240 \\ 
NGC 7217 & 331.968292 &  31.359333 & 0.003176 & 11.0 & 10.1 &  8.9 & --21.8 & 3.9 & 0.82 &  45.3 & 34.2 & 83.0 & 0.413 & 0.86 & 2.0 & 0.3 & Sb & 3 & (R)SA(r)ab;Sy  LINER & 241 \\ 
NGC 7320 & 339.014083 &  33.948111 & 0.002622 & 16.0 & 15.0 & 11.8 & --18.5 & 2.2 & 0.50 &  33.6 & 17.4 & 45.0 & 0.329 & 0.27 & 7.0 & 0.4 & S0 & 0 & SA(s)d         HII & 242 \\ 
NGC 7385 & 342.477458 &  11.608556 & 0.026175 & 13.1 & 12.0 & 11.4 & --24.0 & 1.5 & 0.87 &  37.8 & 15.0 & 36.0 & 0.149 & 0.90 & --5.0 & 0.6 & E2 & 0 & cD;E pec:;     LERG & 243 \\ 
NGC 7457 & 345.249708 &  30.144944 & 0.002815 & 12.1 & 11.2 & 10.8 & --19.7 & 4.3 & 0.53 &  32.1 & 21.0 & 130.0 & 0.205 & 0.25 & --3.0 & 0.3 & E-S0 & 0 & SA(rs)0-? & 244 \\ 
NGC 7479 & 346.236042 &  12.322889 & 0.007942 & 11.6 & 10.9 &  7.7 & --25.0 & 4.1 & 0.76 &  57.3 & 45.0 & 25.0 & 0.161 & 0.06 & 5.0 & 0.3 & SBc & 4 & SB(s)c;LINER   Sy2 & 245 \\ 
IC 5298 & 349.002917 &  25.556694 & 0.027422 & 14.9 & 14.0 & 12.9 & --22.6 & 0.7 & 1.00 & * &  3.6 & 108.0 & 0.265 & 0.55 & 3.0* & * & S? & 4 & LINER;HII;SbrstSy2 & 246 \\ 
NGC 7653 & 351.205667 &  15.275583 & 0.014227 & 13.4 & 12.7 & 12.2 & --21.8 & 1.59 & 0.75 &  18.0 & 13.8 & 132.0 & 0.093 & 0.32 & 3.0 & 0.8 & Sb & 0 & Sb & 247 \\ 
NGC 7674 & 351.986333 &   8.779028 & 0.028924 & 13.9 & 13.2 & 11.8 & --23.8 & 1.1 & 0.91 &  12.6 & 10.8 & 150.0 & 0.101 & 0.53 & 4.0 & 0.5 & SBbc & 4 & SA(r)bc pec;HIISy2 & 248 \\ 
NGC 7714 & 354.058750 &   2.155167 & 0.009333 & 13.0 & 12.5 & 12.0 & --21.1 & 1.9 & 0.74 &  11.1 & 12.6 & 79.0 & 0.153 & 0.47 & 3.0 & 0.5 & SBb/P & 3 & SB(s)b:pec;HII LINER & 249 \\ 
IC 5338 & 354.126792 &  21.146000 & 0.054628 & 15.0 & 13.7 & 13.2 & --23.8 & 1.0 & 0.70 & * & 11.4 & 30.0 & 0.105 & 0.40 & --5.0 & 1.8 & E3 & 0 & cD;E?;BrClG & 250 \\ 
NGC 7731 & 355.371125 &   3.740028 & 0.009627 & 13.5 & 12.8 & 12.7 & --20.4 & 1.4 & 0.79 &  15.3 &  4.2 & 95.0 & 0.153 & 0.52 & 1.0 & 0.7 & SBa & 0 & (R)SBa pec: & 251 \\ 
NGC 7741 & 355.976542 &  26.075611 & 0.002502 & 11.8 & 11.3 & 10.0 & --20.2 & 4.4 & 0.68 &  64.2 & 46.2 & 170.0 & 0.137 & 0.10 & 6.0 & 0.3 & SBc & 0 & SB(s)cd        HII & 252 \\ 
NGC 7742 & 356.065542 &  10.767083 & 0.005547 & 12.4 & 11.6 & 11.3 & --20.7 & 1.7 & 1.00 &  15.0 &  9.6 & * & 0.101 & 0.14 & 3.0 & 0.4 & Sb & 3 & SA(r)b;LINER   HII & 253 \\ 
NGC 7743 & 356.088083 &   9.934083 & 0.005704 & 12.4 & 11.5 & 10.8 & --21.2 & 3.0 & 0.87 &  35.1 & 24.6 & 80.0 & 0.173 & 0.25 & --1.0 & 0.3 & SB0-a & 4 & (R)SB(s)0+     Sy2 & 254 \\ 
NGC 7753 & 356.770125 &  29.483444 & 0.017239 & 12.8 & 12.0 & 11.4 & --23.1 & 3.3 & 0.64 & * & 24.6 & 50.0 & 0.193 & 0.14 & 4.0 & 0.3 & SBbc & 0 & SAB(rs)bc & 255 \\ 
NGC 7785 & 358.829292 &   5.915833 & 0.012702 & 12.6 & 11.6 & 10.9 & --22.9 & 2.5 & 0.52 &  23.4 &  9.0 & 143.0 & 0.165 & 0.85 & --5.0 & 0.4 & E5 & 0 & E5-6 & 256 \\ 
NGC 7798 & 359.856250 &  20.749861 & 0.008016 & 13.0 & 12.4 & 11.7 & --21.1 & 1.4 & 0.93 &  15.3 & 12.0 & 51.0 & 0.145 & 0.13 & 5.0* & * & Sc & 1 & SBc            Sbrst & 257 \\ 
%----
\enddata

%\vspace*{-4mm}
\tablecomments{Our sample of 257 galaxies, sorted by R.A. Unless stated
otherwise, all table entries are taken or derived from NASA/IPAC Extragalactic
Database (NED)\tablenotemark{a}\\
Table 1 is published in its entirety in the online journal. A portion is shown
here for guidance regarding its form and content. \\
(1)\; Same as S18 \\
(2)\; R.A. in degrees and in epoch J2000.0 \\
(3)\; Decl. in degrees and in epoch J2000.0 \\
(4)\; Redshift from NED\\
(5)\; Total $B$-band magnitude from Steinicke 2018 \\
(6)\; Total $V$-band magnitude from Steinicke 2018 \\
(7)\; Total 3.6\,\micron\ magnitude measured using GALFIT (AB mag; see Appendix C for more information)\\
(8)\; (7) + Distance Modulus from (4): not taking into account K-correction \\
(9)\; Major axis in arcminutes \\
(10)\; Axis-ratio \\
(11)\; Effective radius in $r$-band in arcseconds from RC3, but recomputed by
RAJ from log(Ae) after accounting for the fact that the listed Ae values
were diameters, not radii \\
(12)\; Petrosian Half-light radius measured in $V$-band in arcseconds \\
(13)\; Position angle from S18 from North through East\\
(14)\; Foreground Galactic extinction \\
(15)\; Bulge-to-total light ratio measured in 3.6\,\micron\ using GALFIT \\
(16)\; T-type from RC3 or assigned (with `*') based on (18) and (20) \\
(17)\; T-type error from RC3 \\
(18)\; Morphological type from S18 \\
(19)\; Assigned SF/AGN classification based on (20) [0\,=\,Not active, 1\,=\,Starburst, 2\,=\,LIRG, 3\,=\,LINER, 4\,=\,Seyfert 2, 5\,=\,Seyfert 1] \\
(20)\; Morphological and activity classification from NED\\
(21)\; Figure Set number\\
\tablenotetext{a}{The NASA/IPAC Extragalactic Database (NED) is operated by the Jet Propulsion Laboratory, California Institute of Technology, under contract with the National Aeronautics and Space Administration.}}
\label{tab:sample}
\end{deluxetable*}
\normalsize



